A Ladder of Causal Distances

Causal discovery, the task of automatically constructing a causal model from data, is of major significance across the sciences. Evaluating the performance of causal discovery algorithms should ideally involve comparing the inferred models to ground-truth models available for benchmark datasets, which in turn requires a notion of distance between causal models. While such distances have been proposed previously, they are limited by focusing on graphical properties of the causal models being compared. Here, we overcome this limitation by defining distances derived from the causal distributions induced by the models, rather than exclusively from their graphical structure. Pearl and Mackenzie (2018) have arranged the properties of causal models in a hierarchy called the "ladder of causation" spanning three rungs: observational, interventional, and counterfactual. Following this organization, we introduce a hierarchy of three distances, one for each rung of the ladder. Our definitions are intuitively appealing as well as efficient to compute approximately. We put our causal distances to use by benchmarking standard causal discovery systems on both synthetic and real-world datasets for which ground-truth causal models are available. Finally, we highlight the usefulness of our causal distances by briefly discussing further applications beyond the evaluation of causal discovery techniques.

==> 060future_work.tex <==
A straightforward application of causal distances concerns the evaluation of causal discovery methods in comparison to a known gold standard as demonstrated by \Secref{sec:discovery eval}. Furthermore, $\ID$ can be used to train and fine-tune hyper-parameters of causal discovery algorithms using a validation set of data with ground-truth causal models. 

The causal distances also have many other applications. 
For instance, one can cluster causal models with similar answers to causal queries (interventions or counterfactuals). Alternatively, by considering $\OD$ and $\ID$ together, one can quantitatively understand the important cases where two models have similar joint distributions but deviate largely in their responses to interventions. These are the cases where a causal understanding is critical because the joint distributions are greatly warped under interventions.

Furthermore, one can embed causal models into vector spaces based on $\ID$ or $\CD$ as demonstrated by \Secref{sec:geometry}. This could be beneficial for performing structure and parameter search in continuous spaces without discarding the interventional properties of the causal model.

% The causal distances can also be extended to time series. For example, an expected interventional distance between two causal models at time step $t$, $\ID^{t}$, can easily be defined. Then, one can study the expected differences $\{\ID^{t}\}_{t \in [T, T+\tau]}$ within a time interval $[T, T+\tau ]$ aggregated through time or visualized itself as a time series. This could have important practical applications in comparing candidate models of dynamical systems upon which we might perform policy changes, e.g., economic models, climate models, \etc.

Interestingly, $\ID$ can also be used as a measure of the resilience of a system by measuring the expected deviation between the system and itself under small random external modifications. Intuitively, a system is resilient if it does not change much under small unexpected perturbations, i.e., $\ID$ should remain small when $P_I$ has small variance.

% Finally, most causal models currently used as benchmarks (\cf\ \Secref{sec:discovery eval}) have a fairly low number of nodes, and in such cases, our proposed estimates are sample\hyp efficient. When, however, the number of nodes is large, one needs to compare joint distributions of potentially high dimensionality. While in principle any specialized technique to compare high-dimensional distributions may be chosen as $D$, scalability becomes an issue that deserves further investigation.

%Measure of resilience, Sensitivity analysis

%Most causal models currently used as benchmarks (\cf\ \Secref{sec:discovery eval}) have a fairly low number of nodes, and in such cases, our proposed estimates are sample\hyp efficient.
%When, however, the numbers of nodes is large, one needs to compare joint distributions of potentially high dimensionality. While in principle any specialized technique to compare high-dimensional distributions may be chosen as $D$, scalability becomes an issue that deserves further investigation.

%Our distances also have many other applications beyond evaluating causal discovery techniques. For instance, one can cluster causal models with similar answers to causal queries (interventions or counterfactuals). Alternatively, one can embed causal models into low-rank vector spaces based on the $\ID$ or $\CD$ distance as demonstrated by \Secref{sec:geometry}.

%The causal distances such as $\ID$ can be used as loss functions to train causal discovery algorithms and fine-tune hyper-parameters. In particular, it is simple to sample random causal models serving as gold standard from which causal discovery algorithms can trained and evaluated as we did in \Secref{sec:discovery eval} with existing techniques.

%The causal distances can also be extended to time series instead of static graphs. In such case, it is possible to define, for example, an expected interventional distance between two causal networks at time step $t$ $\ID^{t}$. The expected differences $\{\ID^{t}\}_{t \in [T, T+\tau]}$ within a time interval $[T, T+\tau ]$ can be aggregated through time or visualize itself as a time serie.

%Additionally, the causal distances induce equivalence classes of causal models (\Secref{properties}). In order to better understand causality and the properties of causal models, it would be important to characterize these equivalence classes. 

%Finally, characterizing fully the relationship between the single-node and the multi-node versions of the causal distances is left for future work.

==> chato-notes.tex <==
% Simple package for inserting notes
% ChaTo - http://www.chato.cl/
% Wed Aug 19 16:46:46 CEST 2009

\ProvidesPackage{chato-notes}[2009/08/19 ChaTo notes]
\RequirePackage{color,marvosym}

% Colors
\definecolor{MyRed}{rgb}{0.6,0.0,0.0} 
\definecolor{MyBlack}{rgb}{0.1,0.1,0.1} 
\newcommand{\inred}[1]{{\color{MyRed}\sf\textbf{\textsc{#1}}}}

% Frame
\newcommand{\frameit}[2]{
    \begin{center}
    {\color{MyRed}
    \framebox[.9\columnwidth][l]{
        \begin{minipage}{.85\columnwidth}
        \inred{#1}: {\sf\color{MyBlack}#2}
        \end{minipage}
    }\\
    }
    \end{center}
}

\DeclareOption{show}{
	\newcommand{\note}[2][]{\def\@tmpsig{#1}\frameit{{\Pointinghand} Note}{#2\ifx \@tmpsig \@empty \else \mbox{ --\em #1}\fi}}
	\newcommand{\todo}[2][]{\def\@tmpsig{#1}\frameit{{\Writinghand} To-do}{#2\ifx \@tmpsig \@empty \else \mbox{ --\em #1}\fi}}
	\newcommand{\inote}[1]{\inred{$\lceil${{\Pointinghand} }} {\sf #1} \inred{$\rfloor$}}
	\newcommand{\citemissing}[0]{\inred{[citation]}}
}
\DeclareOption{hide}{
	\newcommand{\note}[2][]{}
	\newcommand{\todo}[2][]{}
	\newcommand{\inote}[1]{}
	\newcommand{\citemissing}[0]{}
}

\ProcessOptions

